PipeLLM: Fast and Confidential Large Language Model Services with Speculative Pipelined Encryption

Confidential computing on GPUs, like NVIDIA H100, mitigates the security risks of outsourced Large Language Models (LLMs) by implementing strong isolation and data encryption. Nonetheless, this encryption incurs a significant performance overhead, reaching up to 52.8 percent and 88.2 percent throughput drop when serving OPT-30B and OPT-66B, respectively. To address this challenge, we introduce PipeLLM, a user-transparent runtime system. PipeLLM removes the overhead by overlapping the encryption and GPU computation through pipelining - an idea inspired by the CPU instruction pipelining - thereby effectively concealing the latency increase caused by encryption. The primary technical challenge is that, unlike CPUs, the encryption module lacks prior knowledge of the specific data needing encryption until it is requested by the GPUs. To this end, we propose speculative pipelined encryption to predict the data requiring encryption by analyzing the serving patterns of LLMs. Further, we have developed an efficient, low-cost pipeline relinquishing approach for instances of incorrect predictions. Our experiments on NVIDIA H100 GPU show that compared with vanilla systems without confidential computing (e.g., vLLM, PEFT, and FlexGen), PipeLLM incurs modest overhead (less than 19.6 percent in throughput) across various LLM sizes, from 13B to 175B.

==> archived/analysis.tex <==
\section{Analysis}
\label{sec:analysis}

% [cheng: moved this to preamble.tex]
%\newcommand{\confcompute}{confidential computing}

This section will show and analyze the performance drop
brought by the current NVIDIA confidential computing architecture
in various LLM offloading scenes.
% Like OLAP and OLTP in database systems, LLM could also be used in
% throughput-oriented scene as well as serving scene which is latency-sensitive.
Both model swapping and K/V cache swapping are included in consideration.
Besides model weights and K/V cache, the input and output tokens are also
encrypted in {\confcompute}. We also evaluate the performance impact of
encryption of other data.


\heading{Simulating \nv Confidential Computing.}
\cheng{
    * \nv CC ecosystem is not ready
      * Intel doesn't have the CVM
      * what about AMD + H100?
    * however, \nv's driver is available
    * What we do:
      * read the driver
      * confirm key techniques with \nv people (cites to forum posts)
        %[cheng: may need to hide the link for double-blind]
      * simulate \nv CC by adding overheads
    * What we do:
      * intel + A100
      * XXX
}


\subsection{Case Study: Model Swapping}

% LLM is able to process large datasets.
% In this scene, users prefer throughput to latency.
% Flexgen \cite{flexgen-paper} proposed a system targeting this scene.
% It applies offloading techniques with optimizations to enable
% running models on a single GPU even if their parameter exceeds GPU memory.
LLM inference systems require model swapping mechansism if model size exceeds GPU memory.
Flexgen \cite{flexgen-paper} proposed an inference system that supports model swapping.
It applies offloading techniques with optimizations to enable
running models on a single GPU even if their parameter exceeds GPU memory.
One of the optimizations is overlapping CPU-GPU data transfer and GPU compute by
transferring the next layer of weights while computing the current layer on GPU

We run a opt-66b model upon Flexgen on one A100 GPU with 80GB video memory.
The two models requires about 132GB memory on the GPU respectively to store the weights.
The GPU memory is not enough, so the inference procedure requires offloading to work.

\input{fig-s3}

%\begin{figure}
%    \includegraphics[width=\linewidth]{./figures/analysis-flexgen-opt-66b.eps}
%    \caption{\textbf{Throughput of baseline and emulated CC.}}
%    \textmd{X-axis is configuration of Flexgen.}
%    \label{fig:analysis-flexgen-opt-66b}
%\end{figure}

Figure \ref{fig:analysis-flexgen-opt-66b} shows the performance of inference.
We test two configurations.
The left of the figure is offloading 60\% model weights and the batch size is 8.
The other configuration sets the batch size to 32 while the GPU can only hold 50\% model weights because larger batch size requires more memory for computation.
{\confcompute} brings at most 80\% performance overhead.
This is because CPU-GPU data transfer is the performance bottleneck.
Flexgen uses 24GB/s throughput on PCIe lane, while {\confcompute} is limited to
about 4.5GB/s due to encryption\CP{cite}.
Flexgen has already implemented overlapping,
the encryption bandwidth on CPU degrades its performance.
Larger batch size would increase the compute time per batch,
and has significant performance improvement on baseline,
but the performance on {\confcompute} only improves slightly.

\subsection{Case Study: K/V Cache Swapping}
\label{subsec:analysis-kv}

%\begin{figure}
%    \includegraphics[width=\linewidth]{./figures/analysis-vllm-opt-30b.eps}
%    \caption{\textbf{Latency of baseline and emulated CC.}}
%    \textmd{}
%    \label{fig:analysis-vllm-opt-30b}
%\end{figure}

Even if model size fits in GPU memory,
the dynamic input and output sequence length make it a challenge for K/V cache management
in LLM interactive applications such as chatbots.
% LLM has also been applied in interactive applications such as chatbots.
% These applications are more sensitive to latency,
% so the inference system should keep low latency while gaining high throuput.
vLLM is the state-of-art inference system targeting LLM serving.
It implements K/V cache swapping to handle the dynamic property of input and output token.

We run a OPT-30b model upon vLLM on the same platform as above.
Since vLLM targets LLM serving scene, which is latency sensitive,
we analyze the impact of encryption on latency.
Note that vLLM proposes recompute as an alternative to K/V cache swapping,
but recomputing has not been implemented on advanced decoding algorithms in vLLM.
We evaluate parallel sampling of vLLM, which is one of the most common decoding policies in serving scene.
In this test, each input would generate 4 output sequences.

Figure \ref{fig:analysis-vllm-opt-30b} shows the performance of baseline and {\confcompute} in vLLM test.
In low request rate, the overhead of {\confcompute} 
is not significant.
It is because the K/V cache is enough to hold all requests,
so K/V cache does not require swapping.
It also implies that the overhead of encryption of input/output tokens is negligible.

As the request rate grows, the latency of baseline slightly grows,
because K/V cache swapping occurs.
However, the latency of {\confcompute} grows rapidly because of swapping.
During the procedure of encryption on CPU, the GPU cannot proceed but wait because the input is not ready.
The empty cycles would affect the latency of this request and other pending requests,
which amplifies the overhead on latency.

% \subsection{Why does}
% \label{subsec:analysis-vanilla}

% \noindent\textbf{Model Offloading.}

% \noindent\textbf{K/V Cache Swapping.}

% \subsection{Difference between network I/O and GPU I/O}
% \label{subsec:analysis-diff}

% \noindent\textbf{Data Pattern.}
% Data in network I/O is random.

% \noindent\textbf{CPU Ultilization.}


==> archived/bg.tex <==
\section{Background}
\label{sec:bg}

%\cheng{Yifan, please see my comments below.
%After you fix the content,
%don't delete my comments (you can comment them in ltx).
%I need them to track the fixes.
%}

\subsection{Large language models}
\label{subsec:bg-llm}
\label{ss:llm}
% Goal of this subsection:
% 1. Introduce LLM. How LLM computes? => Part 1: Introduce transformer, self-attention and K/V Cache
% 2. Why swapping/offloading is an important technique? =>
%     Part 2.1: If model size could not fit in GPU
%     Part 2.2: If model size could fit in GPU, dynamic K/V Cache

%\cheng{do prior papers use the work ``offload''? if so, put down a paper link
%for me to refer}
%\yifan{Flexgen uses the term offload: https://arxiv.org/abs/2303.06865, and
%vLLM uses the term swap: https://arxiv.org/abs/2309.06180.}

%\cheng{a note for Yifan; see ltx}
%[cheng: I think we should use "offload" for model and "swap" for cache,
%following the wording convention ]


% Part 1
\heading{Serving LLMs.}
Large language models (LLMs) are a category of neural networks specifically crafted to comprehend, generate, and manipulate human languages.
These models function by taking a sequence of text as input and producing a corresponding sequence of text as output.
The Transformer architecture~\cite{vaswani2017attention} stands as the predominant framework in LLM design:
almost all well-known LLMs uses this architecture, including GPT~\cite{brown2020gpt} and LLaMA~\cite{touvron2023llama}.


%\cheng{here is a logic jump: you talked about transformer and then jump to KV
%cache (is it ``KV'' or ``K/V''?).
%You need some transition to connect the two.}
%\yifan{It's KV cache, instead of K/V cache. I would fix the mistakes.}
%\cheng{Yifan, fillin transition}
An LLM typically comprises an input embedding layer, numerous transformer layers (ranging from tens to hundreds),
and an output embedding layer.
The inference process of an LLM begins with a prompt,
which is a series of tokens or words.
Outputs are then generated in an iterative approach.
In each iteration, the model processes the sequence through all its layers to generate a subsequent token.

More specifically, during the servicing of a user prompt,
the model first interprets the user's input tokens to produce the initial new token.
This token then feeds back to the LLM to generate the following tokens.
This iterative process, known as auto-regressive generation,
persists until producing an end-of-sequence token,
or until the output length reaches a pre-set limit, defined either by the user or the model parameters.

\heading{KV Cache in LLM.}
\label{ss:kvcacheintro}
In the process of generating a new token,
the attention mechanism within LLMs captures the relationship between the current input token and all preceding tokens.
Consequently, the LLM needs to calculate the context of these earlier tokens,
which are represented as key and value vectors.
By storing these vectors into the \emph{\kvcache}~\cite{pope2022kv}, LLMs can bypass repetitive calculations of these vectors,
thus significantly improving the efficiency of inferences.
However, the trade-off for this efficiency improvement is an increase in the GPU memory consumption.

%After a token is generated, the suffix 
%of the sequence (including this token)
%would be used as input in every iteration that follows.
%In transformer layers, massive repetitive computation occurs.
% % Therefore, \kvcache is introduced\CP{by who? cite}
% % to speed up the inference procedure by reusing some of the intermediate result.
% % at the cost of more GPU memory usage.
%While \kvcache greatly reduces computation,
%it occupies considerable GPU memory.
%as large as 3 times of model weights~\cite{pope2022kv}.

%\cheng{here explain what \kvcache is and why it costs extra memory (think of a
%reader who barely know anything)}
%\yifan{should I explain the detail of transformer layers and K/V Cache? My idea
%only uses the regular pattern of LLM, so I just want to emphasize this point.}
% [cheng: now is fine]

% The memory usage of \kvcache of a request could be depicted as:
% \[2 \cdot t \cdot n_{layers} \cdot n_{heads} \cdot h \cdot n_{tokens}\]
%\cheng{explain all the terms (like $t$) here}
%\yifan{the formula of memory usage of \kvcache is not required, so I uncommented it.}

% Part 2.1
\heading{Memory Pressure in LLM.}
The parameter count of Large Language Models (LLMs) has been escalating rapidly to enhance accuracy and generalization capabilities.
For example, OpenAI's GPT-2, released in 2019,
consists of 1.5B parameters, while GPT-3, introduced in 2020, boasts 175B parameters.
In contrast, advancements in GPU memory capacity have been comparatively modest.
The A100 GPU, launched in 2020, offers options of 40GB or 80GB of memory,
and the H100 GPU, released in 2022, comes with 80GB of memory.
Thus, the limited GPU memory has emerged as a significant bottleneck in the efficient serving of LLMs.

The memory pressure associated with Large Language Models (LLMs) originates from two primary sources.
First, the sheer size of LLM models frequently exceeds the available GPU memory capacity.
Second, even when the GPU memory is adequate for the model's parameters,
the dynamic properties of the {\kvcache} introduce additional complexity.
In LLM serving systems, accurately predicting the memory requirement for the {\kvcache}
is challenging due to the varying lengths of input prompts
and the unpredictable output lengths that cannot be determined until the inference process is complete.
For instance, about 30\% of GPU memory is allocated for storing the KV cache~\cite{vllm-paper}.


%It would influence the batch decision:
%the output length is unknown until the model generates the end of sequence token,
%so the inference system could not decide whether batching another request would
%make the \kvcache usage overflow.

\heading{GPU memory swapping.}
To mitigate the challenges of LLM memory pressure,
previous studies have introduced various GPU swapping techniques.
Considering the layer-by-layer characteristics inherent in LLM architecture,
the inference system FlexGen~\cite{flexgen-paper} loads the parameters of the active layer onto the GPU,
while maintaining the parameters of other layers in CPU memory.
Similarly, vLLM~\cite{vllm-paper} addresses memory shortages by temporarily pausing some of the requests in the running batch,
subsequently swapping out its {\kvcache} vectors to free up GPU memory.
These vectors are later reloaded to resume processing.
In multi-GPU configurations, LLMs can distribute model weights and {\kvcache} across various GPUs,
utilizing strategies such as tensor parallelism~\cite{shoeybi2020megatronlm}.
%Although our paper primarily focuses on single-GPU environments, the analyses and observations presented are also applicable to multi-GPU setups.

%We believe 
%Our design also applies to multi-GPU.

\subsection{Confidential Computing}
\label{subsec:bg-cvm}
% Goal of this subsection:
% 1. What new threat does cloud computing bring? => Part 1: Motivation of CVM
% 2. Does CVM introduce new challenge? => Part 2: CVM I/O

\iffalse
% Part 1
While deploying application workload on cloud brings considerable benefits,
it exposes more attack surfaces than running on local machine.
On cloud server, the host gets full control of the machine.
Users' workload on the cloud, whether as processes, containers or VMs,
is totally visible and even modifiable to the host.
Even if the cloud provider is trusted,
recent CVEs reveal that attacker could gain full control of the server with certain approaches.
Once attackers have the same privilege as the server administrator,
they can peek into users' workload to steal privacy-sensitive data such as cryptographic keys,
modify the control flow to produce wrong results or run mining application with users' wallet.
\fi

%\cheng{Prior first paragaph is off the point
%(we shouldn't emphase cloud is insecure/malicious, which will later bite us).
%Instead, you should deliver:
%* cloud computing is super useful for serving LLMs
%* sering LLMs requires confidential (don's say cloud is malicious)
%* condifendital computing can help (cite Azure cloud CC)
%* SGX won't help; CVM is a natural fit for LLMs
%}

Today's LLMs are commonly deployed on servers outfitted with high-end GPUs,
an approach that entails significant financial costs.
Cloud deployment, as an alternative, introduces a pay-as-you-go model,
facilitating elastic GPU utilization and ensuring high availability for LLM services.
Despite these advantages, concerns about privacy,
such as the safeguarding of sensitive LLM model weights and the confidentiality of user data and responses,
remain prevalent among LLM owners and end-users.
Confidential computing emerges as a viable solution to these concerns.
In response, cloud service providers, including Microsoft Azure~\cite{azure-cc,azure-h100cc} and Google Cloud~\cite{googlecloud-cc},
have introduced \emph{confidential virtual machines (CVMs)} as a key measure to address these privacy issues.
CVMs provide robust isolation from untrusted hypervisors,
enhancing security and privacy without requiring significant changes to the existing cloud infrastructure.

%of confidential computing.
%
%SGX, another popular solution of confidential computing,
%does not fit for serving LLMs
%as it requires application modifications and has limited private memory.
%
%because SGX requires modification on application.
%CVM's user-transparency reduces users' effort of deploying their LLM inference
%workload to cloud.

\heading{Confidential VMs (CVMs).}
A CVM, such as Intel TDX~\cite{tdxmodule} and AMD SEV-SNP~\cite{sevsnp},
isolates user's OS (the guest) from hypervisor (the host) and secures user's
code and data without modifying applications.
CVMs rely on hardware assistance,
wherein CPU vendors introduce additional security features.
For example, CVMs use encryption to protect their private memory from
potential external attacks.
One of the greatest advantage of CVMs over other solutions is user transparency:
users' applications do not need any modifications,
owning to transparent hardware features and host/guest kernel supports.
%
%Application code in user mode does not require any modification because
%patches in 
%host kernel and guest kernel 
%have already done the work for supporting CVM.

% Part 2
%Existing work shows that isolation and memory encryption brings little performance overhead
%on CPU computing and memory access.
CVMs generally incur minimal performance overhead,
averaging around 4\%~\cite{sevsnp-perf}.
This efficiency is attributed to hardware extensions\cite{sevsnp, tdxmodule}
and software optimizations~\cite{li2021twinvisor, li2023bifrost}.
However, I/O operations in CVMs introduce substantial performance overheads.
This is primarily due to the intensive data copying and encryption/decryption processing involved in DMA requests~\cite{li2023bifrost}.
In traditional VMs, both the host and devices, with IOMMU configured appropriately,
can directly access the memory of guest VMs in para-virtualized and passthrough I/O modes, respectively.
In contrast, CVMs have to use shared IO buffers to prevent the host from accessing CVM memory
and require end-to-end encryption of IO data, both of which result in significant overheads.

%CVM's isolation and memory encryption build a wall between the guest and host
%for security, but it in turn hurts I/O performance.
%

%

%In current hardware, the communication happens at shared memory of guest VM,
%at which device drivers should place the data for I/O, bringing additional
%penalty on performance.
%Furthermore, because attackers on the host can read and write the shared memory,
%the I/O data has to be encrypted ahead of transfer.
%Encryption of I/O data cannot reuse CVM's memory encryption and would use
%end-to-end encryption cipher, which hurts the performance even worse due to
%poor performance of end-to-end encryption on CPU. CPU vendors have planned to
%introduce new hardware features (e.g., Intel TDX Connect and AMD TIO) to enable
%devices access CVM private memory just like in traditional VM. However, no
%hardware (including CPU and device) supports it currently. This work targets
%existing hardware that uses shared memory and end-to-end encryption for I/O.

%\subsection{Confidential Computing on GPUs}
\label{subsec:bg-h100}

%\cheng{Yifan, write a paragraph of confidential GPUs in academia including the
%recent software-based ones.}

\heading{Confidential Computing on GPUs.}
In addition to CPU-side CVMs, the concept of confidential computing
extends to the GPU domain,
offering effective protection for LLMs against untrusted hypervisors.
Soter~\cite{atc2022soter} presents a system designed for edge computing scenarios
that relies on CPU-side confidential computing,
thereby eliminating the need to trust the GPU hardware.
This system leverages a technique known as parameter morphing,
which enables the offloading of layers with associativity properties to GPUs.
This approach ensures that the plaintext of model weights remains secure and undisclosed to untrusted GPUs.
But Soter has large overhead (2$\times$ to 15$\times$) on LLM inference tasks
because non-associative layers, such as the embedding layers,
has to be computed on CPUs.
Honeycomb~\cite{osdi2023honeycomb} adds a trusted software component
and uses static validation the block insecure commands to GPUs before submitting them.
Honeycomb requires extra runtime checks for indirect memory access
which is intensively used in LLM inference systems like vLLM~\cite{vllm-paper},
bringing non-trivial performance overhead.
% Example: The layer is y = k * x + b. The CPU sends 2 * k and 2 * b to the GPU,
% And compute the layer on the GPU, and then divide the result by 2.
% Drawback of Soter

%
% Honeycomb


% Goal of this subsection: Introduce H100 confidential computing
Unlike software-based solutions,
\nvcc relies on hardware:
\nv H100 GPU is the first commercial implementation with confidential computing
capability~\cite{h100cc-paper}.
Working with CVMs, H100 could build a GPU enclave, allowing user to have
exclusive control over the GPU and rejecting any access from host, such as
read/write GPU memory and modify the control flow.
Hardware GPU \cc has low performance overhead
and is backward-compatible with existing applications.
This paper focuses on studying hardware GPU \cc.





\iffalse
[cheng: note for me

current flow:
 - LLM intro
 - memory is the bottleneck
   -- solution: swapping
     -- model
     -- kv-cache
 - CVM
 - confidential GPUs
]

\fi


==> archived/design.tex <==
\section{Design}
\label{sec:design}

\newcommand{\prediction}{prediction\xspace}
\newcommand{\predict}{predict\xspace}
\newcommand{\encworker}{encryption worker\xspace}
\newcommand{\allocation}{ciphertext placement\xspace}
\newcommand{\bounce}{bounce ciphertext placement\xspace}
\newcommand{\zerocopy}{zero-copy ciphertext placement\xspace}
\newcommand{\inplace}{inplace ciphertext placement\xspace}

\subsection{\sys Prediction}
\label{subsec:design-prediction}

%\heading{Swapping data \prediction.}
%\TODO{Use another term to replace prediction}
\sys's predictor predicts which memory chucks to be swapped and their IVs.
%
The predictor focuses on major GPU memory swaps---model weights offloading and
\kvcache swapping.
Other than the two, I/Os %DMAs
also involve other small data transfers,
for example, user input and output tokens.
As mentioned in section~\ref{sec:analysis},
since the encryption of them bring negligible overheads,
\sys does not pipeline them.
% \sys predicts data swapping based on the swapping history.
% The size of model layer and K/V cache have some relation and feature,
% so whether a request is model weights or K/V cache can be implyed based on the size.
By the model definition (i.e., its computational graph and weights),
\sys distinguishes the data of model weights and KV cache with high accuracy
without additional hints from LLM applications.
% \sys identifies parameters when they are allocated on or loaded into GPU.
Therefore, \sys can distinguish the data of model weights and \kvcache with
high accuracy without additional hints from LLM applications.
Therefore, \sys knows if a memory swap is model offloading
or \kvcache swapping with high confidence.

\begin{figure}
    \subfloat[Layer-wise prediction] {
        \includegraphics[width=0.5\linewidth]{./figures/drawio/design-prediction-layer.pdf}
        \label{fig:design-predict-layer}
    }
    \subfloat[Request-wise prediction] {
        \includegraphics[width=0.5\linewidth]{./figures/drawio/design-prediction-request.pdf}
        \label{fig:design-predict-request}
    }
    \vspace{1ex}
    \caption{\textbf{Prediction of \sys}}
    % \textmd{X-axis is configuration of FlexGen.}
    \label{fig:design-predict}
\end{figure}

%\heading{IV \prediction.}
% Model weight offloading in LLM training or inference systems typically follows a consistent pattern,
% making the offloading trace identical among iterations and predictable for \sys.
% The model can either be fully offloaded or partially offloaded (where part of the model is offloaded).
% In the case of full offloading, the process adheres to the layer-by-layer structure of model execution.
% In partial offloading, LLM applications typically offload the same set of parameters across iterations
% given that each transformer layer has identical structure and size
% For example, if an application offloads parameters from layers 1 and 3 in one iteration,
% it will likely continue to offload these specific layers in subsequent iterations.
% This consistency makes the offload pattern highly predictable for \sys.
% Therefore, for model offloading,
% \sys tracks the offloading history of all offloaded blocks.
% Later, \sys predicts an IV and pre-encrypts the upcoming blocks of parameters.
% \sys learns whether the model is in forward or backward pass, adapting to the sequential and reverse sequential patterns, respectively.
For model offloading, \sys monitors swapped layers from the start of the application,
maintaining a swap history to predict the next layer to be reloaded.
Figure \ref{fig:design-predict-layer} gives an example:
\sys identifies a pattern where parameters from layer 1 are first swapped out, followed by layers 3 and 4, and then back to layer 1.
This pattern indicates that layers 1, 3, and 4 are offloaded to the CPU.
Layer 2, not appearing in the swap history and computed immediately after layer 1 due to the layer-by-layer nature of LLMs, is therefore not offloaded.
Similarly, other layers are also not offloaded.
Given that the most recent layer in the swap history is layer 1,
\sys predicts that layer 3 will be the next to be reloaded and prepares it with an appropriate IV for encryption.
The swap history for model offloading in most applications typically follows a circular pattern, as illustrated in this example.
Since each layer shares the same structure and number of parameters,
it is unlikely that applications will offload a particular layer in some iterations while retaining it in the GPU during other iterations.
This consistency results in the same layers being offloaded across multiple iterations.
%
% For K/V cache swapping, {\sys} currently accepts linear patterns (FIFO and LIFO).
% It works for the cases in the evaluation part.
% More patterns are explored in the future.

\kvcache swapping is typically conducted on a layer-wise or request-wise basis, both of which are highly predictable patterns.
In layer-wise swapping, the application decides whether to swap the \kvcache generated in each layer for all requests in the batch.
Alternatively, request-wise approach involves swapping all layers of \kvcache from certain requests in case of memory shortage to free up memory for others.
Layer-wise swapping aims to achieve high throughput as it allows the batch size to remain unchanged.
Othervise, request-wise swapping reduces latency for high-priority requests and lowers the average latency overall.
% ecause \kvcache is private to a certain request and can not be used by other requests.
Layer-wised swapping follows a consistent pattern and is highly predictable for \sys.
% For \kvcache swapping, the swapping policies
% of existing systems---for example, Flexgen~\cite{flexgen-paper},
% vLLM~\cite{vllm-paper} and DeepSpeed~\cite{deepspeed-paper}---are
% either FIFO or LIFO.
% This makes sense, as the swapped \kvcache is either layer-wised---swapping
% \kvcache of each layer in order, hence FIFO---or
% associates with requests:
% swapping out all \kvcache for one user request.
% Request-based swapping is likely to be LIFO 
% because the first swapped-out request has the lowest priority, so it is swapped in last.
% \sys learns the current swapping pattern and predicts near-future swaps by
% following the pattern.
% For example, if the policy is FIFO and memory chucks are
% swapped out in the order of \texttt{chunk A}, \texttt{chunk B}, and \texttt{chunk C};
% \sys then pre-encrypt in the order of \texttt{chunk A, B, C} with corresponding IVs.
%
In request-wise \kvcache swapping, applications usually swap out the lowest priority request in the current batch when facing a memory shortage.
Consequently, the first request to be swapped out is likely the one with the lowest priority among the swapped requests, and it will be the last to be reloaded.
\sys can learn and predict this pattern with a high degree of accuracy.
Note that \sys's approach applies to other regular \kvcache swapping policies,
and can be easily extended to future systems.

\subsection{Ciphertext Validation}
\label{ss:s5-validation}

Before sending ciphertext with a specific IV to the GPU,
\sys must verify that it matches the data intended for the loadback operation by LLM applications.
% A simple verification method involves storing the plaintext of the predicted loadback blocks and performing a byte-level comparison with the data used in the loadback operation.
% However, this method's overhead increases proportionally with the data size, leading to significant inefficiencies.
One possible \(O(1)\) approach involves storing the address range of predicted loadback blocks and comparing it with the actual loadback operation.
This \(O(1)\) method is effective for swapped blocks when applications do not modify them.
However, if an application retrieves some data from the GPU, updates the values in-place after \sys's encryption on the old data, and then writes the entire block back to the GPU, this method could result in sending ciphertext of outdated data.
Such a scenario involving those data compromises the system's correctness.
\sys builds its validation method based on the \(O(1)\) validation approach
with page protection mechanism from virtual memory.
The validation works as follows.
%
During the prediction stage, \sys labels each pre-encrypted ciphertext with
the corresponding plaintext's address range on the CPU memory.
%
\sys then revokes the write permission of these memory pages.
% \sys revokes the write access of application on the predicted data range.
%
Therefore, when facing data modifications by the application,
%prediction errors\CP{why prediction errors}
%or applications writing to the memory,
\sys detects the changes by a page fault.
The page protection can thus prevent \sys from violating the system's correctness.
%
During validation stage at runtime, \sys checks if the address and length
of the swap %response
align with the associated labels to determine the match between plaintext
and ciphertext.
This method is generally highly effective for LLMs
because applications do not move or update the swapped model weights or \kvcache in the CPU memory.

\begin{figure}
    \includegraphics[scale=0.5]{./figures/drawio/cipher-validation.pdf}
    \caption{Ciphertext validation.}
    \textmd{\sys only records the base addresses and sizes of swapped data blocks.
    The validation checks the two, consuming \(O(1)\) time.
    Application's write to predicted swapped blocks means the prediction is wrong.}
    \label{fig:design-cipher-validation}
\end{figure}
% \TODO{A figure to describe ciphertext validation}

% It is implemented by MPK/PKU for thread-level protection.

\subsection{Tolerating wrong IVs with Re-ordering and Padding NOPs}
\label{subsec:nop-insertion}

% Re-order example:
% Prediction block number: 1 2
% Request block number: 2 1
%% Request block 2 => prediction larger than current, pending
%% Then, request block 1 => prediction ok
It can happen that LLM applications reload some data blocks at a certain IV,
but \sys predicts at a IV higher than current.
% The opposite case would not happen because \sys drops predictions whose IVs are smaller than current for old IVs are never used in the future.
It is noticable that LLM applications may swap multiple blocks together. \TODO{Mention it earlier}
In this case, a synchronize call would be triggered by the applications marking the finishing boundary of swapping.
Using this feature, \sys would first pend a swapping request with wrong IV,
and re-order disjoint swapping requests to match the predicted IV.
Thanks to the efficient validation time, the pending brings little overhead.

% NOP example:
% Prediction block number: 1 2
% Request block number: 2
% \sys: NOP => swap 2 and drop 1 (actually, predict 1 at a higher IV)
After re-ordering, there might still be some pending requests, which is solved by padding NOPs in the design of \sys.
A 1-byte data could be send to increase the current IV with small overhead,
and \sys could ultilize the predicted ciphertext without re-encryption even if the predicted IV is larger.

\TODO{Discussion: Re-ordering does not bring overhead.
1 NOP costs 10us, while reencrypting 1MB costs 232us.
\sys can combine those two methods.}

\begin{figure}
    \includegraphics[scale=0.5]{./figures/drawio/tolerate-wrong-iv.pdf}
    \caption{Tolerate wrong IVs.}
    \label{fig:design-tolerate-wrong-iv}
    \textmd{\sys uses re-ordering requests and padding NOPs to tolerate wrong IVs.
    In this figure, next IV is 1 but the application swaps the block that is predicted to be swapped at iv 3.
    \sys would pend this request until a synchronize request from the application.
    The system's IV would grow with successful predictions.
    At synchronize request, \sys would send NOPs to increase the IV, and invalidate the prediction at the corresponding IV.
    Upon reaching the predicted IV of some pending swapping request, \sys would commit it.}
\end{figure}
% \TODO{A figure of Tolerating wrong IVs}

\iffalse
\subsection{Tolerating IVs with Padding NOPs}
\label{subsec:nop-insertion}

All I/Os between confidential VMs and GPUs are encrypted,
and each of them requires one IV (\S\ref{ss:iv}).
There are many small-sized I/Os (e.g., user input/output tokens)
that \sys does not pipeline, but they consume IVs.
%
To tolerate these small-sized I/Os,
\sys assigns larger IVs than the predictions,
leaving enough IVs for small-sized data requests that happen
in-between memory swaps.
%
For example, if the IV for the next predicted
swapped data is $2000$, \sys produces a slightly larger IV like $2100$.
%
During the validation,
if the current IV (say $2070$) is smaller than
the IV used for pre-encryption (that is $2100$),
\sys pads \emph{NOP transfers} until the used IV ($2100$) is current.
A NOP is a 16-byte piece of data,
where 16-byte is the minimum unit for AES encryption.
%
If no predicted ciphertext occupies the IV, the 16-byte data is dummy;
otherwise, \sys encrypts the first 16 bytes of the predicted
plaintext. %\CP{later, too encoded}
%
These 16-byte NOPs are copied to the same destination as the request,
which will later be replaced by the actual requested data.
%
This approach enables \sys tolerating small-sized data
transfers without compromising the confidentiality and integrity of the
inference process.
\fi

\iffalse
% \noindent\textbf{NOP insertion.}
% \TODO{Padding NOP (current IV is less than predicted IV)}
% Although small-size DMAs (such as input and output tokens) does not affect the performance of {\confcompute}, it highly affects the predictor.
% {\sys} should reserve the space of the counter for potential small-size DMAs.
% {\sys} uses 16-byte transfer (minimum unit of AES encryption algorithm) to increment the IV on the GPU.
% If the minimum predicted IV is larger than current IV, the 16-byte is filled with 0.
% Else, the 16-byte is the first 16-byte of predicted ciphertext to avoid information leak.
% The destnation address is the last DMA of this tranfer to be covered.
\sys ultilizes small-sized data transfers to solve the problem brought by dynamic small-sized data transfers during the inference.
In the prediction stage, \sys ensures that the predicted IV leaves ample space for small-sized data requests from the application.
For instance, the IV for the next predicted swapped data is slightly larger than the current IV.
During the validation stage, if the plaintext requested by the application corresponds to some ciphertext,
but the predicted IV exceeds the current IV, \sys can execute 16-byte transfers,
the minimum unit for AES encryption, to increment the current IV until it aligns with the predicted IV.
These 16-byte transfers are directed to the same destination as the request,
allowing padding data to be replaced with meaningful data.

If no predicted ciphertext occupies the IV, the 16-byte data can be arbitrary.
Othervise, \sys would choose the first 16 bytes of the predicted plaintext.
This approach ensures that PipeInfer efficiently handles small-sized data transfers without compromising the confidentiality and integrity of the inference process.
\yifan{Padding NOP makes IV prediction more flexible. If data prediction works and succeeds, predicting a larger IV would not bring overhead to this transfer.
The drawback is, the ciphertext using the padding IVs has to be dropped.
The re-prediction and encryption is overlapped during this transfer and the next transfer.}
\fi

\subsection{Asynchronous Decryption}
\label{ss:asyncdecrypt}

% The prediction module accelerates CPU-to-GPU data transfer of \cc.
% For eliminate the overhead of CPU-side decryption on GPU-to-CPU data transfer,
% \sys leverages asynchronous decryption.
% First, \sys detects whether the transferred belongs to \kvcache
% (note that the GPU does not modify the model weights, so the swapped model weights are
% directly dropped instead of copied to CPU).
% Based on the observation that CPU does not modify the \kvcache,
% To detect and handle prediction failure, \sys disables the read and write permission
% of the application threads on those data.
% On prediction error, and the application tries to read or write that data,
% an page fault would trigger and \sys would synchronously decrypt the data
% and then continues the execution of the application.

% The following is by chatgpt: [cheng: no longer true]
%\cheng{Yifan, please check if the following description is true}
%\yifan{Yes.}

So far, we mostly talked about CPU-to-GPU data transfers and CPU-side encryption.
For CPU-side decryption during GPU-to-CPU data transfers,
We found that LLM applications do not modify swapped data except during the swapping process.
Other data may be processed on CPU after being loaded from the GPU.
Based on this observation, \sys employs asynchronous decryption for swapped data.
It returns the memory copy API before decryption and leaves the memory at the destination address unchanged.
%
It works as follows.
\sys determines whether the data being transferred is part of the \kvcache or model parameters
based on their feature on data size mentioned earlier.
If yes, \sys decrypts it asynchronously for better overlapping;
otherwise, \sys does the default, decrypting the data immediately.
%based on our observation of classifying swapped data (\S\ref{ss:observation}).
%%% In training, GPU might modify the weights
% It's important to note that the GPU
% does not modify the model weights; therefore, any swapped model weights
% are simply discarded rather than copied back to the CPU memory.
% This implies that large-sized transfers are very likely to be \kvcache.
%
At mis-prediction, the applications may process the data before decryption.
To detect usage-before-decryption,
\sys revokes the read and write permissions of the application for
the plaintext which is a placeholder before decryption finishes.
%based on the observation that the CPU does not alter the \kvcache,
If the application attempts to
access (read or write) this data, a page fault occurs.
\sys then decrypts the data synchronously and allows the application to
continue its execution.


\subsection{Side-Channal-Free Ciphertext Placement}
\label{subsec:design-allocation}

\TODO{Divide into shared memory management and private memory management}

Current cuda uses zero-copy placement: the cipher text is computed in CVM shared memory.
In our design, using zero-copy placement would expose ciphertext that would not be commited, leading to potential side channel.
Therefore, \sys store the ciphertext in private memory like bounce buffer.
To eliminate the memory copy and metadata handle overhead,
\sys leverages fix-sized buffers in shared memory for DMA to eliminate memory allocation in critical path
and pipelines data copy with PCIe transfer.
Because memory copy is faster than PCIe, the pipeline does not require much buffer for the memory copy stage,
minimizing the usage of CVM shared memory.

\sys limits the private memory usage by an encryption window.
The window size is configured based on application behaviors,
for example, when facing model offloading, the window is set to be the size of the next layer.
The memory of ciphertext in the window would not be released until the prediction is commited, or dropped due to prediction errors.

%If faced with memory shortage, \sys uses inplace placement to let ciphertext occupy the memory of plaintext.

%\TODO{Specify}

\iffalse
\sys allocates memory on confidential VMs (CVM) to store ciphertexts.
%produced by \encworker.
CVM hardware limits the DMA region within shared memory of the guest
VM, so the data must be placed somewhere before DMA.
This particularly a problem for  \sys, as it does the encryption in advance
and needs to manage the ciphertext in memory.
% {\sys} proposes three policies, based on trade-offs on the following concerns:
%
Next, we describe two \allocation policies used by existing CVM systems,
and introduces two optimized policies we propose.
Figure \ref{fig:design-cipher} depicts the four polices,
showing how and when the plaintext is encrypted,
and its allocation in CVM private memory or shared memory.

% \begin{itemize}
%     \item Performance on prediction success. It is highlighted when nearly all prediction succeeds.
%     \item Penalty on prediction failure. Even with high precition success rate, handling prediction failure brings extra overhead and hurts the tail latency of {\sys}.
%     \item Resource usage. CPU resource is costly in cloud. LLM offloading requires hundreds of GBs of memory, so memory usage should also be restricted.
% \end{itemize}

% \begin{figure}
%     \includegraphics[scale=0.8]{./figures/design-cipher-in-private.pdf}
%     \caption{Basic memory placement.}
%     \label{fig:design-cipher-in-private}
% \end{figure}

\iffalse
\begin{figure}[t]
    \includegraphics[scale=0.9]{./figures/design-cipher.pdf}
    \caption{\CF{\allocation} policies.
    Each light orange box depicts a policy.
    Purple boxes refer to ciphertext allocated in CVM private memory;
    orange boxes refer to ciphertext allocated in CVM shared memory;
    and green boxses refer to plaintext (always allocated in CVM private memory).
    Data marked with ``temp'' can be freed by the runtime or driver.
    The boxes below box ``APP'' belong to applications' address space,
    and the boxes below box ``Runtime'' are in the runtime or driver's address space.
    Solid arrows refer to operations after application sends the copy command
    and are always in the critical path,
    and dashed arrows refer to predictive operations and can be pipelined.}
    \label{fig:design-cipher}
\end{figure}
\fi


%\heading{\bounce.}
% This policy takes the bounce buffer mechansism as reference.
% The encrypted data is stored in CVM private memory.
% On DMA launch, a temporary buffer is allocated in shared memory and
% the encrypted data is copied to there.

% This policy involves an additional memory copy in critical path of every DMA, compared with baseline.
% It would bring performance overhead.
% On the other hand, it hides the ciphertext in the private memory,
% and is flexible in handling prediction failure.

\iffalse
\heading{\CF{\bounce}.}
Linux (as guest VM) kernel-mode driver adopts the bounce buffer mechanism.
The first dashed box in figure \ref{fig:design-cipher} shows its procedure.
After the application calls memory copy to GPU,
the runtime or driver encrypts the data to another place in CVM private memory,
and then copies the data to CVM shared memory for DMA.
The two ciphertext buffers can be freed directly after the DMA finishes.
The additional copy would bring non-negligible performance overhead\cite{li2023bifrost}.

% \begin{figure}
%     \includegraphics[scale=0.8]{./figures/design-cipher-in-shared.pdf}
%     \caption{Zero-Copy memory placement.}
%     \label{fig:design-cipher-in-shared}
% \end{figure}

\heading{\CF{\zerocopy}.}
This policy allocates the ciphertext in shared memory, shown in the second
dashed box in figure \ref{fig:design-cipher}.
It reduces the memory copy of {\bounce}.
% Therefore, it would not bring performance overhead compared to baseline on prediction success.
% {\sys} uses this mode for weights swapping and adds encryption window for low memory usage
% (for example, only encrypt the next layer for model weights prediction).
This policy is used in current NVIDIA driver \cite{nvidia-driver}
% \yifan{Should I reference the github repo of nvidia driver code?}\cheng{YES}.
However, zero-copy does not work for \sys because
% \cheng{Yifan, fillin what is wrong}
it introduces potential cache attack, leaking sensitive data.
(we describe the details in the security analysis, \S\ref{ss:securityanalysis}.)
\fi

% This policy exposes ciphertext before the data is confirmed to transfer.
% Therefore, upon prediction failure, it has some limitation compared to {\bounce}.
% Using one IV for encrypting multiple plaintext would leak the key to attackers.
% To increment the IV on the GPU, the CPU has to launch DMA,
% which occupies the PCIe lane.

% \begin{figure}
%     \includegraphics[scale=0.8]{./figures/design-cipher-in-self.pdf}
%     \caption{Cipher text in original place.}
%     \label{fig:design-cipher-in-self}
% \end{figure}

\heading{Windowed ciphertext placement.}
This is one policy used by \sys when memory is abundant.
\sys adopts similar design to {\bounce}, shown in the third box in
Figure~\ref{fig:design-cipher},
but the copy part can be pipelined with prediction without overhead on the critical path.
\sys uses an encryption window for memory usage.
The window size is configured based on application behaviors,
for example, when facing model offloading, the window is set to be the size of the next layer.
The memory of ciphertext in the window would not be released until it is copied
to GPU or dropped due to prediction errors.

\heading{\CF{\inplace}.}
This is another policy used by \sys when memory is limited.
When an application requires a large window,
the above windowed policy can consume substantial memory,
potentially impairing the performance of the inference system.
To address this issue, \sys introduces \emph{inplace encryption}.
This method discards the plaintext and replaces it with ciphertext,
as depicted in the fourth dashed box in Figure~\ref{fig:design-cipher}.
During prediction, this approach decrypts the ciphertext,
and re-encrypts the data using the predicted new IV.
To be secure,
inplace encryption requires two additional copies
to avoid attacks described in the zero-copy policy.
This policy effectively reduces memory usage
at the cost of additional memory copies and longer latencies.
%increased CPU time for encryption processes.
%
Furthermore, under this policy, the application is unable to directly access
the plaintext. When the application accesses the plaintext, a page fault
is triggered, prompting \sys to restore the data by decrypting on-the-fly.
%This approach is particularly
%employed when the guest VM's current memory usage exceeds a certain threshold.
\fi
% The above two policies require more memory to store the ciphertext.
% This policy does not store the plaintext of data.
% Instead, it only stores the ciphertext.
% To generate the ciphertext based on the next predicted IV,
% it requires decrypting the stored ciphertext first,
% and then does the encryption.

% Compared with the other two policies,
% this policy saves memory because it does not keep the plaintext version of predicted data.
% However, it requires twice CPU resources as the other two.
% Upon prediction failure, it also brings more performance overhead.

% Replace by ChatGPT version below
% {\sys} uses this mode for K/V cache swapping because of high predicion accuracy.
% If the application requires a large window, the windowed policy consumes a lot of memory,
% which potentially hurts the performance of the inference system.
% To solve this problem, {\sys} proposes inplace encryption,
% which drops the plaintext and covers it by the ciphertext,
% shown in the fourth dashed box in figure \ref{fig:design-cipher}.
% Upon prediction, this policy first decrypts the ciphertext using the old IV,
% and then encrypts the data using the predicted new IV.
% This policy reduces the extra memory usage, at the cost of doubled CPU time for encryption.
% Furthermore, application could not read the plaintext from this address,
% so when it happens, a page fault should be triggered to let \sys recover the data.
% This policy is used when the VM's current memory usage is beyond a threshold.



% \subsection{Encryption Workers}
% \TODO{This subsection is about multi-thread.}
% {\sys} allocates encryption workers.

% Trade off between worker num and time

% \subsection{NOP Insertion}

% When prediction is not correct.

% \subsection{Handle Data Modification}

% Application may modify the pre-encrypted data.

% Use page fault mechansism. Disable the read/write permission of user thread.

% \subsection{Encryption Window}

% Save memory usage

% \TODO{It is tuning part. Not mechansism.}


==> archived/overview.tex <==
\section{Overview}
\label{sec:overview}

\subsection{Goal}
\label{subsec:ov-goal}

The primary goal of this work is to eliminate the overhead of Nvidia Confidential Computing, 
while keeping the security guarantees and user transparency.

\subsection{Threat Model}

{\sys} aims at protecting the confidentiality and integrity of LLM applications, model weights, and request and response tokens.
{\sys} adopts similar threat model as Nvidia confidential computing and previous work on GPU confidential computing.
The attacker could have whole control and even physical control over the host system.
\TODO{Briefly introduce the thread model: CPU-side, GPU-side, CPU-GPU data transfer}
DOS attack and side channel attack is out of scope.

\subsection{Main Idea}
{\sys} proposes speculative pipelined encryption so that the encryption is removed out of the critical path.
It predicts the data to be transferred in the near future based on the applications' previous behaviors,
and makes best effort to ensure that the ciphertext to be transferred is ready before applications submit the transfer.

\subsection{Definition of Prediction Success and Failure}

The user asynchronously submits a set of memory copy commands: \(\{t_1, t_2, ..., t_n\}\).
We can assume that the commands do not overlap because of the asynchronous property.
The predictor prepares an ordered sequence of ciphertext: \((p_1, p_2, ..., p_m)\).
\(t\) and \(p\) refers to truth and prediction respectively.

We define the success as:
\[m \ge n\ and\ \{t_1, t_2, ..., t_n\} = \{p_1, p_2, ..., p_n\}\]

Note that the order of \((p_1, p_2, ..., p_n)\) does not make sense because any two commands do not overlap.

\noindent\textbf{F1: data loss.}
\[\exists i \in [1, n], t_i \notin (p_1, p_2, ..., p_m) \]
The preditor fails to predict the swapped data \(t_i\).

\noindent\textbf{F2: wrong sequence.}
The prediction does not meet the condition of prediction success, and \[\{t_1, t_2, ..., t_n\} \subseteq \{p_1, p_2, ..., p_m\}\]

\subsection{Challenges}
There are three main challenges.

\noindent\textbf{C1: predict accurately without user-provided knowledge.}
As a prediction-based system, {\sys}'s performance improvement relies on high prediction accuracy.
One possible approach is to provide extra API for application to guide the prediction.
However, it requires modification to the application and violates the goal of {\sys}.
Therefore, {\sys} should make prediction based on limited knowledge,
including LLM feature and API trace of applications.

\noindent\textbf{C2: handle prediction failure.}
The prediction system could not ensure 100\% accuracy.
Even with high accuracy, {\sys} should have a mechanism for prediction failure.
On one hand, the failure handling should be fast to avoid high tail latency.
On the other hand, attackers may potentially obtain information from the failure data and the transferred data,
so it should avoid leaking sensitive information to attackers.

\noindent\textbf{C3: hardware resource is limited.}
\TODO{This is an abstract idea. CPU and memory}
Additional CPUs.
Offloading technology in LLM consumes lots of memory, so {\sys} should limit its memory usage.

\subsection{Obseration}
\noindent\textbf{O1: LLM swapping feature.}
% Two features: layer-by-layer, and generative by GPU.
Read-only swapping (model weights, GPU does not modifies the weights)
and dirty swapping (K/V cache, all K/V cache is generated by GPU).

\noindent\textbf{O1.1: LLM layer-by-layer feature.}
For read-only swapping of model weights, {\sys} can use the layer-by-layer feature of LLM inference.
The application would not move the model weights on the CPU to another place of memory.
{\sys} could predict memory address of the next layer to be transferred.

\noindent\textbf{O1.2: LLM K/V Cache feature.}
For dirty swapping, CPU would not modify the swapped data;
the swapped data has to be swapped in to finish an inference request.
This paves the way for high accuracy prediction.

\subsection{Architecture}
\begin{figure}
    \includegraphics[width=\linewidth]{./figures/overview-arch.pdf}
    \caption{\textbf{Overview of {\sys}}}
    % \textmd{X-axis is configuration of Flexgen. \TODO{More configurations.}}
    \label{fig:overview-arch}
\end{figure}

Based on the observations, we propose {\sys}.
Figure \ref{fig:overview-arch} shows the architecture of {\sys}. 
{\sys} works on the library and driver level, requiring no modification to user applications.
{\sys} is composed of prediction modules, failure handle module and memory allocation module.
The prediction module has high accuracy of the set of based on the observations.
We found that \textbf{F1} is hard to solve but rarely exists because of the observations,
so the failure handle module is optimized to solve \textbf{F2}.
Memory allocation is proposed to minimize the memory usage of {\sys}.
Encrption window and inplace encryption is proposed based on \textbf{O1.1} and \textbf{O1.2} respectively.

% \subsection{Challenges}

% \TODO{The challenges are not suitable.}

% \noindent\textbf{C.1 Encryption cannot be avoided.}

% \noindent\textbf{C.2 Complexity of various LLM applications.}

% \subsection{Obseration and Insight}

% \noindent\textbf{O.1 Regular pattern I/O.}

% \noindent\textbf{O.2 ML framework.}

% \subsection{Architecture}

% To handle the above challenges, we propose \noindent\textbf{predictive encryption at system level}.

% \subsection{Threat Model}

% \TODO{Move to above}
